Importance Weighting Can Help Large Language Models Self-Improve

Large language models (LLMs) have shown remarkable capability in numerous tasks and applications. However, fine-tuning LLMs using high-quality datasets under external supervision remains prohibitively expensive. In response, LLM self-improvement approaches have been vibrantly developed recently. The typical paradigm of LLM self-improvement involves training LLM on self-generated data, part of which may be detrimental and should be filtered out due to the unstable data quality. While current works primarily employs filtering strategies based on answer correctness, in this paper, we demonstrate that filtering out correct but with high distribution shift extent (DSE) samples could also benefit the results of self-improvement. Given that the actual sample distribution is usually inaccessible, we propose a new metric called DS weight to approximate DSE, inspired by the Importance Weighting methods. Consequently, we integrate DS weight with self-consistency to comprehensively filter the self-generated samples and fine-tune the language model. Experiments show that with only a tiny valid set (up to 5\% size of the training set) to compute DS weight, our approach can notably promote the reasoning ability of current LLM self-improvement methods. The resulting performance is on par with methods that rely on external supervision from pre-trained reward models.

==> sections/Limitation.tex <==
\section*{Limitation}
Limited by time and computing resources, our work has two major weakness.

First, the base model (Llama3-8B) used in experiments is not very strong. This affects the quality of self-generated samples. Whether using samples generated from a more powerful model would undermine the significance of incorporating importance weighting needs further experiments and discussion.

The other limitation is the naive approximation of importance weights (Eq.~\ref{equ:weight-est}). While this method is computationally efficient, it may lead to estimation errors because of ignoring the semantic similarity among samples. We expect training a model to predict the importance weight would be a better estimation approach and leave it for future work.
% Although the calculation is computationally cheap, it may introduce estimation error because of ignoring the semantic similarity among samples. We expect training a model to predict the importance weight would be a better estimation approach and leave it for future work.

==> tables/weak2strong.tex <==
\begin{table}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lccc}
    \toprule
     & base & Qwen1.5-1.8B & Llama3-8b \\
    \midrule
    gsm8k & 6.8 & - & 37.6 \\
    SVAMP & 14.7 & 56.3 & 62.7 \\
    ANLI-A1 & 16.4 & 27.4 & 27.2 \\
    ANLI-A2 & 14.6 & 24.0 & 22.4 \\
    OpenBookQA & 31.8 & 49.2 & 37.0 \\
    StraregyQA & 48.3 & 50.9 & 54.59 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Weak2Strong.}
    \label{tab:w2s}
\end{table}
